Efficient $k$-Clique Listing: An Edge-Oriented Branching Strategy

$k$-clique listing is a vital graph mining operator with diverse applications in various networks. The state-of-the-art algorithms all adopt a branch-and-bound (BB) framework with a vertex-oriented branching strategy (called VBBkC), which forms a sub-branch by expanding a partial $k$-clique with a vertex. These algorithms have the time complexity of $O(k m (\delta/2)^{k-2})$, where $m$ is the number of edges in the graph and $\delta$ is the degeneracy of the graph. In this paper, we propose a BB framework with a new edge-oriented branching (called EBBkC), which forms a sub-branch by expanding a partial $k$-clique with two vertices that connect each other (which correspond to an edge). We explore various edge orderings for EBBkC such that it achieves a time complexity of $O(\delta m + k m (\tau/2)^{k-2})$, where $\tau$ is an integer related to the maximum truss number of the graph and we have $\tau < \delta$. The time complexity of EBBkC is better than that of VBBkC algorithms for $k>3$ since both $O(\delta m)$ and $O(k m (\tau/2)^{k-2})$ are bounded by $O(k m (\delta/2)^{k-2})$. Furthermore, we develop specialized algorithms for sub-branches on dense graphs so that we can early-terminate them and apply the specialized algorithms. We conduct extensive experiments on 19 real graphs, and the results show that our newly developed EBBkC-based algorithms with the early termination technique consistently and largely outperform the state-of-the-art (VBBkC-based) algorithms.

==> cover-letter/meta.tex <==
\section*{Comments from Meta-Reviewer}


\begin{enumerate}[leftmargin=*,itemindent=0.6cm]

    \smallskip
    \item[O1.] \textit{Highlight novelty of iterating over edges instead of vertices.}

    \smallskip
    \begin{response}
        We have highlighted (1) the novelty of edge-oriented branching based framework (see our responses to R1O1 and R2O1) and (2) the potential applications our new method to more cohesive subgraph mining problems (see our response to R3O1).
        % {\yuiR We highlight novelty of iterating over edges (i.e., \texttt{EBBkC} vs \texttt{VBBkC}) from the following points.
        % \begin{itemize}[leftmargin=*]
        %     \item \emph{Theoretical gains} (R2O2, R3O3). 
        %     Recall that \texttt{EBBkC} and \texttt{VBBkC} run in $O(km(\tau/2)^{k-2})$ and $O(km(\delta/2)^{k-2})$, respectively. 
        %     The theoretical gain (i.e., the gap between $\delta$ and $\tau$) is significant in most graphs, as newly discussed in Section~\ref{subsec:EBBkC-T}.
        %     \item \emph{Practical performance gains} (R4O1(1,2)). \texttt{EBBkC} (without early termination) runs faster than \texttt{VBBkC} methods, as verified in the newly added experiments in Section~\ref{subsec:result} 
        %     (3).
        %     \item \emph{Potential extensions} (R3O1). \texttt{EBBkC} can be potentially extended to solve other graph mining tasks, as newly discussed in Section~\ref{subsec:discussion}.
        % \end{itemize}
        % }
        %We highlight the novelty of iterating over edges instead of vertices as follows. By iterating arbitrary edge ordering, any instance of \texttt{VBBkC} can be covered by an instance of \texttt{EBBkC}, but not vice versa. This further explains why the instance of \texttt{EBBkC} with the truss-based edge ordering can achieve a better worst-case time complexity. 
        %
        %Details refer to R1O1 and R2O1. 
    \end{response}

    
    \smallskip
    \item[O2.] \textit{Highlight that despite the complexity improvement is not phenomenal, experimental results have shown significant improvements.}

    \smallskip
    \begin{response}
        We have highlighted (1) the theoretical improvement (in terms of time complexity) can be significant (see our responses to R2O2, R3O3 and R4O2) and (2) empirical improvements are clear and consistent (see our responses to R4O1(1,2,5)).
        % {\yuiR
        % We clarify the complexity improvement and the experimental improvement as follows.
        % \begin{itemize}[leftmargin=*]
        %     \item \emph{Complexity improvement} (R2O2, R3O3). The complexity improvement (i.e., the gap between $\delta$ and $\tau$) is significant in the most real graphs, as newly discussed in Section~\ref{subsec:EBBkC-T}.
        %     \item \emph{Experimental improvement} (R4O1(1,2)). The experimental improvement is more significant since both the \texttt{EBBkC} framework and the early termination (which does not improve the theoretical time complexity in our analysis) contribute to the improvement and the later contributes more, as verified in the newly added experiments in Section~\ref{subsec:result} (3). %(note that the early termination does not improve the complexity). 
        % \end{itemize}
        % } 
        %We clarify the reason of the improvements as follows. We first note that the improvements mainly come from two key components: (1) the Edge-oriented Branch-and-Bound (EBB) framework and (2) the early-termination technique. Although in some graphs, when the complexity improvement is not phenomenal (i.e., $\tau$ is close to $\delta$), we observe that there always exists an abnormally large clique (e.g., an 82-clique in \textsf{WE}, an 87-clique in \textsf{CI} and a 114-clique in \textsf{DB}). In this case, our early-termination technique can recognize these cliques during the enumeration and thus significantly reduce the running time. 
        %
        %Details refer to R2O2 and R3O3. 
    \end{response}


    \smallskip
    \item[O3.] \textit{Add experiments as suggested in the reviews.}

    \smallskip
    \begin{response}
        We have added the following experiments.

        \begin{itemize}[leftmargin=*]
            \item \emph{Ablation studies} for showing the contributions of the edge-oriented branching framework and the early termination technique (Section~\ref{subsec:result} (3)). See our responses to R4O1(1,2) for details.
            
            \item \emph{Time for generating truss-based edge ordering and degeneracy ordering} (Section~\ref{subsec:result} (3)). See our response to R4O1(6) for details.
            
            \item \emph{Space costs} (Section~\ref{subsec:result} (8)). See our responses to R3O2 and R4O2(3) for details.
            
            \item \emph{Scalability test} (Section~\ref{subsec:result} (9)). See our responses to R4O1(4) for details.
            
        \end{itemize}
        
    \end{response}

\end{enumerate}



==> cover-letter/review1.tex <==

\section*{Comments from Reviewer \#1}

\begin{enumerate}[leftmargin=*,itemindent=0.6cm]

    \smallskip
    \item[O1.] \textit{The core solution is a seemingly simple extension of the vertex-based approach. Specifically, the main difference is that, instead of considering candidate ones one at a time at each branching step, the proposed solution considers them in pairs, as long as they are already connected by an edge. Indeed, when the same configurations are used for both approaches (Fig. 5), the relative performance difference is much less pronounced. As such, it may be better for the authors to reposition their paper as general improvements to VBBkC, as opposed to an altogether new framework.}

    \smallskip
    \begin{response}
    Thank you for your comment. We tend not to position our \texttt{EBBkC} as an improvement within the \texttt{VBBkC} framework since any instance of \texttt{VBBkC} can be covered by an instance of \texttt{EBBkC}, but not vice versa. This is because for \texttt{EBBkC}, we can explore arbitrary edge orderings for each branching step, while for \texttt{VBBkC}, the underlying edge orderings (via two branching steps) are constrained by the vertex ordering that is adopted. For example, the instance of \texttt{EBBkC} with the truss-based edge ordering (i.e., \texttt{EBBkC-T}) corresponds to no instance of \texttt{VBBkC}.
    \end{response}


    \smallskip
    \item[M1.] \textit{Referring to ``vertices that connect/disconnect a vertex to/from some graph'' is a bit confusing.}

    \smallskip
    \begin{response}
         %We have changed ``connect'' to ``connect with'' or ``adjacent to'' and changed ``disconnect'' to ``not connected with'' or ``not adjacent to'' accordingly.
      We have changed ``disconnect'' to ``is/are disconnected from''.
      % , as suggested in R4D3.
       % We rewrote those sentences and marked them in blue in the revised manuscript. 
    \end{response}
    

    
    \smallskip
    \item[M2.] \textit{It would be good if the authors could further provide definitions of the concepts used in this work (e.g., degeneracy, k-truss, etc.).}

    \smallskip
    \begin{response}
    We have included the definition of degeneracy in Section~\ref{sec:intro}. The $k$-truss concept is not used in the paper and thus its definition is not provided explicitly.
    % {\yuiR We have included the definitions in Section~\ref{sec:problem}.}
       %Thanks for the suggestion. We provided such definitions in Section 2. 
    \end{response}
    
    
    \smallskip
    \item[M3.] \textit{The introductory section gives examples of graphs where the proposed solution might find uses, most of which are directed and weighted graphs. Section 2 changes the scope to unweighted and undirected graphs. It would be good if the two were better matched.}

    \smallskip
    \begin{response}
    As we have checked, in those applications mentioned in the introduction, when $k$-clique listing is performed, the weights and directions of graphs (if any) are ignored. The weight and direction information (if any) is used in other components involved in those applications.
    % We carefully checked the applications that mentioned in the introduction and found that when the $k$-clique listing is a key component for some other problems, they often first regard the graph as unweighted and undirected, and use the weights or the directions for the downstream tasks. Therefore, we can assume that the input graph is undirected and unweighted. 
    \end{response}
    
    
    
    \smallskip
    \item[M4.] \textit{It is a bit unclear how the algorithm detects whether $g$ transforms into a $t$-plex for some $t$.}

    \smallskip
    \begin{response}
        We check the minimum degree of a vertex in $g$ - if it is no less than $|V(g)|-t$, $g$ is a $t$-plex; otherwise, $g$ is not a $t$-plex. 
       % We can determine whether $g$ is a $t$-plex for some $t$ by checking whether the minimum degree of a vertex in $g$ is no less than $|V(g)|-t$, which can be done simultaneously when constructing the corresponding branch $B=(S,g,l)$ in at most $O(V(g))$ time.
        %
       We have included the above details in Section~\ref{sec:early-termination}.
       
       %We included how the algorithm detects whether $g$ is $t$-plex for some $t$ in Sec.~\ref{sec:early-termination}. 
    \end{response}


    \smallskip
    \item[R1.] \textit{I would like to thank the authors for their responses. My main consideration with this work is its novelty over the vertex-based BB k-clique approach. The core idea is that a "k-clique can be constructed by merging a clique S and an l-clique, where |S| + l = k. VBBKC consider 1-cliques (l=1) and the current work considers 2-cliques, but both are covered by the overarching framework. As a side-note, from a high-level point of view I don't see how this alone can lead to the complexity gains proposed in the paper; there is the potential for pruning a larger part of the search space earlier with EBBKC, but there is also a much larger number of l-cliques to consider. Figure 5 seems to indicate that the two approaches are not that far off wrt performance, once some satellite ideas have been applied to both. It makes one wonder whether the huge performance boosts seen in other figures are down to engineering and dataset details, but the complexity analysis provided by the authors indicates that some improvements in performance should be expected. Furthermore, following up on comment R3O2, it would be good to know the raw numbers from the experiments, not just the big-O complexity analysis.}

    \smallskip
    \begin{response}
        \underline{First}, our \texttt{EBBkC} algorithm improves over the \texttt{VBBkC} algorithms in terms of theoretical time complexity. Empirically, both the edge-oriented BB framework and the early termination technique contribute to the improvement over \texttt{VBBkC} algorithms. We refer to our response to R4O1(1,2) for details. \underline{Second}, we have reported the empirical space costs in Section~\ref{subsec:result} (8). The results show that the empirical space costs of all methods are comparable, which is consistent with our theoretical big-O complexity analysis.
    \end{response}

\end{enumerate}


==> cover-letter/review2.tex <==

\section*{Comments from Reviewer \#2}

\begin{enumerate}[leftmargin=*,itemindent=0.6cm]

    \if 0
    \smallskip
    \item[O1.] \textit{Niche focus.}
    
    \smallskip
    \begin{response}
        We address this concern from the following aspects. 
        %
       \underline{First}, our framework can be easily adapted to solve other clique mining tasks, including Maximal Clique Enumeration (MCE), Maximum Clique Search (MCS) and Diversified top-$k$ Clique Search (DCS). The rationale is that our framework can explore all possible cliques in an input graph and thus can output only the desired cliques that satisfy some property (e.g., maximality and diversity) by filtering out others.
       %
        \underline{Second}, our framework can be potentially extended to mining other types of \textit{connected} dense subgraphs, e.g., connected $k$-plex. This is because our framework can be used to explore all possible subsets of edges by recursively including an edge, and thus the induced subgraphs will cover all possible connected dense subgraphs.
        %
        \underline{Third}, there are some potential benefits when adapting our framework to the above tasks. As discussed in Section~\ref{subsec:motivation}, the edge-oriented branching provides us more information (i.e., an edge involving two vertices instead of one vertex) towards designing more effective pivot techniques and/or pruning rules than the existing vertex-oriented branching.
        %
        We include the above discussions in our revised manuscript.
    \end{response}
    \fi

    \smallskip
    \item[O1.] \textit{Niche focus and incremental work. }

    \smallskip
    \begin{response}
       We emphasize that the idea of edge-oriented branching is not an incremental idea as it looks to be. We explain as follows. There is a vast literature of branch-and-bound (BB) algorithms for various graph data mining problems (including the $k$-clique listing problem that we target in this paper). To the best of our knowledge, these algorithms all adopt the vertex-oriented branching strategy, i.e., they take it for granted that BB algorithms should form branches by including a \textit{vertex} each time. In our paper, we deviate from this approach for the first time and form branches by including an \textit{edge} each time. Our idea is novel and cannot be found in any of the existing BB algorithms. Furthermore, it is an interesting finding that with some appropriate edge ordering, the BB algorithm based on our edge-oriented branching can improve the time complexity of the state-of-the-art BB algorithms based on vertex-oriented branching. Lastly, our edge-oriented branching can potentially be adapted to solve other subgraph mining tasks (see our responses to R3O1 for details), which we plan to explore as future research directions.
    \end{response}

    \smallskip
    \item[O2.]  \textit{Theoretical gains are not always significant since $\tau$ can be very close to $\delta$ for many graphs. As $k$ increases also gains become minimal.}

    \smallskip
    \begin{response}
       \underline{First}, for an input graph with $n$ vertices, we can prove that the gap between $\tau$ and $\delta$ can be as large as $n/2$ (i.e., it can be infinity theoretically) and the ratio of $\tau/\delta$ can be as low as 0.
       %
        \underline{Second}, the ratio $\tau/\delta$ is below 0.8 for the majority of the datasets we used (15 out of 19). $\tau$ and $\delta$ are close on 4 datasets only, namely \textsf{WE}, \textsf{CI}, \textsf{DB} and \textsf{UK}. This is because there exists an abnormally large clique in these datasets (e.g., an 82-clique in \textsf{WE}, an 87-clique in \textsf{CI}, a 114-clique in \textsf{DB} and a 944-clique in \textsf{UK}), which results in the proximity of $\tau$ to $\delta$. For example, in the 114-clique within DB, every vertex has 113 neighbors (which implies that $\delta=113$) and every pair of vertices has 112 common neighbors (which implies $\tau=112$).
        %
        \underline{Third}, we have collected the statistics of the gap on 139 more real-world graphs (\url{http://lcs.ios.ac.cn/~caisw/Resource/realworld%20graphs.tar.gz}) and found that the ratio is below 0.8 for the majority (105 out of 139).
        %
        \underline{Fourth}, our algorithms runs $(\delta/\tau)^{k-2}$ times faster than the state-of-the-art (i.e., $O(km(\tau/2)^{k-2})$ v.s. $O(km(\delta/2)^{k-2})$). When $\tau/\delta$ is at most 0.8 (which holds for most of the datasets) and $k = 12$, the speedup of our algorithm is at least ${1.25}^{10}=9.31$, which is already about an order of magnitude.
        %
        We have included the above discussions in Section~\ref{subsec:EBBkC-T}.
    \end{response}

    \smallskip
    \item [D1.] \textit{Clarification on Figure 4.}

    \smallskip
    \begin{response}
        \underline{First}, the zoomed-in parts in Figure 4 of the original version (now Figure~\ref{fig:real-large}) are to better distinguish the lines when $k$ is small or near $\omega$; \underline{Second}, we  omit the results for some values of $k$ since the time costs are beyond 24 hours due to the large number of $k$-cliques. We have included the above clarifications in Section~\ref{subsec:result} (2).
        %We shall provide the above clarifications and improve the presentation of in a revision (see Sec.~\ref{subsec:setup} and Sec.~\ref{subsec:result} (2)).

    \end{response}
    
\end{enumerate}

==> cover-letter/review3.tex <==

\section*{Comments from Reviewer \#3}

\begin{enumerate}[leftmargin=*,itemindent=0.6cm]

    \smallskip
    \item[O1.] \textit{The $k$-clique listing problem has received substantial attention within the academic literature. Consequently, it could be beneficial to delve deeper into the following facets: (1) Could the framework potentially be expanded to encompass tasks beyond exhaustive enumeration, such as diversified enumeration? For instance, consider the reference \cite{yuan2016diversified} as an illustrative example even if addresses cliques. (2) Is there potential for this framework to be extended to address other challenges involving dense subgraphs?}

    \smallskip
    \begin{response}
       Thanks for the comment. 
       % We list some of the possible directions that our framework can be extended to address as follows. 
       Our \texttt{EBBkC} framework can be potentially applied to other problems than the $k$-clique listing problem, which we discuss as follows.
       %
       \underline{First}, our framework can be easily adapted to solve other clique mining tasks, including Maximal Clique Enumeration (MCE), Maximum Clique Search (MCS) and Diversified top-$k$ Clique Search (DCS). The rationale is that our framework can explore all possible cliques in an input graph and thus can output only the desired cliques that satisfy some property (e.g., maximality and diversity) by filtering out others.
       %
        \underline{Second}, our framework can be potentially extended to mining other types of \textit{connected} dense subgraphs, e.g., connected $k$-plex. This is because our framework can be used to explore all possible subsets of edges by recursively including an edge, and thus the induced subgraphs will cover all possible connected dense subgraphs.
        %
        \underline{Third}, there are some potential benefits when adapting our framework to the above tasks. As discussed in Section~\ref{subsec:motivation}, the edge-oriented branching can provide more information (i.e., an edge involving two vertices instead of one vertex) towards designing more effective pivot techniques and/or pruning rules than the existing vertex-oriented branching. 
        We plan to explore these directions as future work.
        %
        We have included the above discussions in Section~\ref{subsec:discussion}.
    \end{response}

    \smallskip
    \item[O2.] \textit{How does the new approach impact memory usage? Please provide experimental results.}

    \smallskip
    \begin{response}
        The space complexity of our \texttt{EBBkC} algorithm is $O(m+n)$, which is the same as those of the existing methods. We have included space complexity of our \texttt{EBBkC} algorithms in Theorem~\ref{theo:ebbkc-t}, Theorem~\ref{theo:ebbkc-c} and Theorem~\ref{theo:ebbkc-h}.
        We have reported the empirical space costs in Section~\ref{subsec:result} (8). The results show that the empirical space costs of all methods are comparable, which is consistent with our analysis.
    
       %Thanks for the comment. We have reported the memory usage in Figure~\ref{fig:mem}, {\yuiR and also included the following note in Section~\ref{subsec:result} (8) to explain the results: 
       %
      % ``First, the memory usage of all algorithms is comparable and a few times larger than the graph size, which is aligned with the space complexity of $O(n+m)$. Second, \texttt{EBBkC+ET} has the memory usage slightly larger than the others  since it employs extra data structures for maintaining edge ordering and/or conducting early-termination.''}
       %\texttt{EBBkC+ET} consumes slightly more memory than the existing algorithms but the memory usage is still linear to the size of the graph. The reason is that (1) \texttt{EBBkC} framework produces more branches at each branching step and (2) additional spaces are needed to store the data structures for early-termination. 
       %
       %We included the above descriptions in Sec.~\ref{subsec:result} (8). 
    \end{response}

    \smallskip
    \item[O3.] \textit{$\tau$, as compared to $\delta$, presents a less intuitive concept. To enhance clarity, the paper would benefit from the following additions: (1) More characterization of $\tau$, elaborating more on the definition and adding illustration. (2) Insights on properties leading some graphs to have substantially smaller $\tau$ than $\delta$ and practical applications.}

    \smallskip
    \begin{response}
       The parameter $\tau$ of a graph refers to the largest integer such that there exists a non-empty subgraph where every pair of vertices incident to an edge inside has at least $\tau$ common neighbors. Similar to the degeneracy $\delta$, $\tau$ measures the density of a graph, say, the larger the value of $\tau$, the denser the graph. For an input graph, $\tau$ is always smaller than $\delta$ as it imposes stricter constraints on connections (i.e., every pair of vertices has at least $\tau$ common neighbors vs. every vertex has at least $\delta$ neighbors). Besides, for more discussions on the gap between $\tau$ and $\delta$, please refer our response to R2O2.
       %
       We have included the above discussions on the definitions and insights of $\tau$ in Section~\ref{subsec:EBBkC-T}.
    \end{response}
    
\end{enumerate}

==> cover-letter/review4.tex <==

\section*{Comments from Reviewer \#4}

\begin{enumerate}[leftmargin=*,itemindent=0.6cm]

    \smallskip
    \item[O1.] \textit{Experimental study not sufficiently convincing. }
    % \begin{itemize}[leftmargin=*]
        % \item[(1)] 
        \textit{\underline{(1)} It's not sufficiently clear whether improvements come from edge-based brand-and-bound or solely from early termination. In fact, comparing Fig. 8 with Fig. 3 seems to suggest that the proposed method is slower than prior work without early termination.}
        % \item[(2)] 
        \textit{\underline{(2)} The results of Fig. 5 do not help to clarify, since the VBB method used there does not seem to be a SOTA method (and, in fact, it's unclear which one has been used). }
        % \item[(3)] 
        \textit{\underline{(3)} The \texttt{BitCol} paper \cite{yuan2022efficient} lists lower runtimes than shown in this study (on the same datasets). This mismatch does not seem to be accounted for by different processors (seems to be close). }
        % \item[(4)] 
        \textit{\underline{(4)} The \texttt{BitCol} paper reports results on much larger/more challenging graphs (ClueWeb09, Wikipedia13, AllWebUK02); these should be included here as well, perhaps dropping some of the easy graphs. }
        % \item[(5)] 
        \textit{\underline{(5)} Again, on BitCol, the paper proposes two preprocessing techniques that reduce cost significantly. The last three points together imply that the relative performance w.r.t. \texttt{BitCol} remains unclear. }
        % \item[(6)] 
        \textit{\underline{(6)} What's the time of the truss decomposition? Has it been included? }
        % \item[(7)] 
        \textit{\underline{(7)} The optimal choice of $t$ for each dataset and choice of $k$ is something one cannot do in practice. This should be avoided. }
        % \item[(8)] 
        \textit{\underline{(8)} The runtime of Fig. 10 do not seem to be consistent with the runtimes of Fig. 4. The parallel version is much slower than the sequential one. }
        
    \smallskip
    \begin{response}
       \begin{itemize}[leftmargin=*]
        \item[(1,2)] 
        We note that both the edge-oriented BB (EBB) framework and the early termination technique contribute to the improvement of \texttt{EBBkC+ET}.
        % we conduct the following new experiment in Section~\ref{subsec:result} (3).
        To see this, we revise the experiment in Section~\ref{subsec:result} (3) as follows.
        
        % We compare different versions of \texttt{EBBkC+ET}
        We compare two variants of our method, 
        namely \texttt{EBBkC+ET} (the full version) and \texttt{EBBkC} (the full version without the early termination), with two vertex-oriented BB (VBB) algorithms, namely \texttt{DDegCol+} (the \texttt{DDegCol} algorithm with pruning Rule (2) proposed in this paper) and \texttt{BitCol+} (the \texttt{BitCol} algorithm with pruning Rule (2) and without SIMD-based implementations).
        We note that \texttt{DDegCol+} and \texttt{BitCol+} correspond to the SOTA VBB algorithms without SIMD-based implementations.
        % All these algorithms have not utilized SIMD and thus we rule out \texttt{BitCol} and \texttt{SDegree} for fair comparison. 
        We report the results in Figure~\ref{fig:variant} and have the following observations. 
        \underline{First}, \texttt{DDegCol+} and \texttt{BitCol+} have very similar running times, which shows that pre-processing techniques in the \texttt{BitCol} paper are not effective (we shall provide some explanations in our responses to R4O1(3) and R4O1(5)). \underline{Second}, \texttt{EBBkC} runs clearly faster than \texttt{DDegCol+} and \texttt{BitCol+}, which demonstrates the clear contribution of our EBB framework (note that \texttt{EBBkC} and \texttt{DDegCol+} differ only in their frameworks). We note that it is not fair to compare \texttt{EBBkC} with \texttt{BitCol} directly since the latter is based on SIMD-based implementations while the former is not. \underline{Third}, \texttt{EBBkC+ET} runs clearly faster than \texttt{EBBkC}, which demonstrates the clear contribution of the early termination technique. For example, on dataset \textsf{WK}, the EBB framework and the early-termination contribute 28.5\% and 71.5\% to the efficiency improvements over \texttt{BitCol+} when $k=13$, respectively.
        % First, both \texttt{EBBkC} and \texttt{EBBkC+ET} outperform \texttt{DDegCol+} and \texttt{DDegCol++}, which verifies the effectiveness of EBB framework and the early termination technique. Second, \texttt{EBBkC+ET} performs the best and runs significantly faster than \texttt{EBBkC}. This demonstrates that the early termination technique contributes more to the practical improvement of \texttt{EBBkC+ET}. Third, \texttt{DDegCol+} and \texttt{DDegCol++} achieves the similar performance and run slightly faster than \texttt{DDegCol}, for which we believe they are the SOTA except \texttt{BitCol} and \texttt{SDegree}. 
        
        % {\kaixinB
        %\underline{First}, for the setting, we choose \texttt{DDegCol} (as VBB algorithm) and \texttt{EBBkC} (as EBB algorithm). Both algorithms (1) employ all color value-based pruning rules and (2) rule out early-termination technique and SIMD. In this case, \texttt{DDegCol} differs with \texttt{EBBkC} only in the framework. Besides, we also add a baseline \texttt{DDegCol+}, which is based on \texttt{DDegCol} and further enables two pre-processing in \cite{yuan2022efficient}. In this case, \texttt{DDegCol+} is the state-of-the-art VBB baseline without SIMD. 

        
        %\underline{Second}, for illustration, we combine Figure 9 in the original paper to the Figure~\ref{fig:variant} to show the contribution of each component to the practical speedups, respectively. We note that the early-termination technique contributes more to the practical speedups than the EBB framework. For example, on dataset \textsf{WK}, the EBB framework and early-termination contribute 28.5\% and 71.5\% to the efficiency improvements, respectively. 
        % as verified in Figure~\ref{fig:variant} {\kaixinB( see the comparison among red, magenta and blue lines). Also, the early-termination technique contributes more to the practical speedups than the EBB framework.}
        
        %\underline{Third}, we note that \texttt{EBBkC} (our algorithm without the early-termination technique) runs slightly slower than \texttt{BitCol}. This is mainly because \texttt{BitCol} enables SIMD for acceleration while \texttt{EBBkC} does not. Hence, the comparison between \texttt{EBBkC} and \texttt{BitCol} is not fair. 
        % We note that the performance \texttt{EBBkC} can be potentially boosted with SIMD-based implementations, which we leave as future work. 
        % }
        
        
        % In particular, experimental results in Figure~\ref{fig:variant} validates the superiority of the EBB framework and the details refer to the response to R\#4O1.(1).
        %
        % Besides, we note that \texttt{EBBkC} without the early-termination technique (in Figure 9) runs slightly slower than \texttt{BitCol} (in Figure 4) on WK and PO. This is mainly because \texttt{BitCol} enables SIMD for acceleration while \texttt{EBBkC} does not. Hence, the  comparison is not fair and thus rarely show the improvements of the EBB framework. We also note that \texttt{EBBkC+ET} runs faster than \texttt{BitCol} on WK and PO, which suggests that the early-termination technique contributes to more practical speedups compared to the EBB framework. 
        
        %All descriptions and experimental results are shown in Exp.~(3) and Figure~\ref{fig:variant}.
        % }
        
        %We clarify the concern from two perspectives. 
        %
        %\underline{First}, we improve our presentation of the comparison between \texttt{VBBkC} and \texttt{EBBkC} by using all state-of-the-arts techniques, including two pre-processing techniques proposed in \cite{yuan2022efficient}, all color value based pruning rules and early-termination technique. We note that both algorithms under \texttt{VBBkC}  and \texttt{EBBkC} do not use SIMD for acceleration for the sake of the fairness. We included the above descriptions in our revised manuscript (see Sec. 6.2 (3)). 
        %
        %\underline{Second}, we admit that the algorithm \texttt{EBBkC-H} without SIMD cannot outperform \texttt{BitCol} when comparing Fig.~\ref{fig:early} with Fig.~\ref{fig:real-small}. But \texttt{EBBkC-H} outperforms other \texttt{VBBkC} algorithms that do not utilize SIMD. We believe that the gap between \texttt{EBBkC-H} and \texttt{BitCol} can definitely be filled if \texttt{EBBkC-H} is also implemented with SIMD. 

        % \item[(2)] 
        % {\kaixinB
        % For the setting, we choose \texttt{DDegCol} (as VBB algorithm) and \texttt{EBBkC} (as EBB algorithm). Both algorithms (1) employ all color value-based pruning rules and (2) rule out early-termination technique and SIMD. In this case, \texttt{DDegCol} differs with \texttt{EBBkC} only in the framework. Besides, we also add a baseline \texttt{DDegCol+}, which is based on \texttt{DDegCol} and further enables two pre-processing in \cite{yuan2022efficient}. In this case, \texttt{DDegCol+} is the state-of-the-art VBB baseline without SIMD. 
        % The results are shown in Figure~\ref{fig:variant}. On dataset \textsf{WK}, for example, the EBB framework and early-termination contribute 28.5\% and 71.5\% to the efficiency improvements when $k=13$, respectively. 
        % }
        % {\yuiR We clarify that the VBB method \texttt{VBBkC+ET} used in Figure~\ref{fig:variant} is the SOTA among all those without using SIMD.
        % %
        % Specifically, \texttt{VBBkC+ET} is based on \texttt{DDegCol} while further employing the pre-processing techniques proposed in~\cite{yuan2022efficient}, all color value based pruning rules and early-termination technique proposed in our paper. Hence, \texttt{VBBkC+ET} differs with \texttt{EBBkC+ET} only in the BB framework.
        % %
        % Note that we rule out \texttt{BitCol+ET} for comparison since \texttt{BitCol} further enables SIMD for acceleration which makes the comparison unfair. 
        % %
        
        % We have included the above notes in Section~\ref{subsec:result} (3).
        % }
        %In Fig.~\ref{fig:variant}, \texttt{EBBkC} differs from \texttt{VBBkC} only in the framework. Both algorithms use two pre-processing techniques proposed in \cite{yuan2022efficient}, all color value based pruning rules and early-termination technique, while both algorithms do not use SIMD. Furthermore, the vertex orderings used in \texttt{VBBkC} follow \texttt{DDegCol} \cite{li2020ordering} and \texttt{BitCol} \cite{yuan2022efficient} by first using degeneracy ordering to branch the universal search space and using color ordering to branch the produced sub-search space. In this case, the algorithms for comparison are both the state-of-the-art. 

        \item[(3)] Based on our checking on the source code of the implementation of \texttt{BitCol}(\url{https://github.com/zer0y/k-clique-listing}), which was provided by the authors of the \texttt{BitCol} paper \cite{yuan2022efficient}, we explain as follows.

        % \underline{First}, 
        The running time results reported in \cite{yuan2022efficient} do not cover the time costs of (1) conducting the pre-processing techniques (i.e., \textit{Pre-Core} and \textit{Pre-List}) and (2) generating the degeneracy orderings for \texttt{BitCol}. Nevertheless, both (1) and (2) are operations involved in the \texttt{BitCol} algorithm, and thus their time costs should have been covered. In contrast, the running times of all algorithms reported in our paper include the time costs of (1) conducting the pre-processing techniques (if any) and (2) generating orderings of vertices.
        
        We have included the above clarification in the experimental setting of Section~\ref{subsec:setup}.  
        
        %We carefully checked \cite{yuan2022efficient} and found the same datasets are \textsf{pokec}, \textsf{dblp} and \textsf{stanford}. The differences mainly come from \textsf{pokec}. According to the implementation of \texttt{BitCol} (which can be found via \url{https://github.com/zer0y/k-clique-listing}), there are two issues that possibly caused the inconsistency. 
        %
        %\underline{First}, for both \texttt{SDegree} and \texttt{BitCol}, their codes do not include the running time of pre-processing to the total running time. This is not reasonable since two proposed pre-processing techniques (\textit{Pre-Core} and \textit{Pre-List}) are both dependant on the value of $k$. 
        %
        %Furthermore, for \textit{Pre-List}, the implementation only counts the $k$-cliques in a clique-like connected component in a combinatorial manner (which only needs $O(1)$ time) instead of listing them (which needs $O(\tbinom{n}{k})$ time if the connected component has $n$ vertices). 
        %
        %\underline{Second}, for both \texttt{SDegree} and \texttt{BitCol}, their codes do not include the running time of generating the orderings (i.e., degree ordering for \texttt{SDegree} and degeneracy ordering for \texttt{BitCol}). For example, on \textsf{pokec}, it needs 7.3 seconds to generate a degeneracy ordering. 
        %
        %In our paper, we reported the time of \texttt{SDegree} and \texttt{BitCol} by fixing all the above issues. 
        
        

        \item[(4)] In the revision, we have included in Table~\ref{tab:data} the suggested larger datasets, namely \textsf{ClueWeb09 (CW)}, \textsf{Wikipedia13 (WP)}, \textsf{AllWebUK02 (UK)}, and reported the experimental results on these newly added datasets in Figure~\ref{fig:scale} and Section~\ref{subsec:result} (9). We note that \texttt{EBBkC+ET} can significantly improve the efficiency when $k$ is near the size of a maximum clique. Notably, on the largest graph \textsf{WP}, \texttt{EBBkC+ET} runs near two orders of magnitude faster than the SOTA algorithm \texttt{BitCol} when $k=425$.
        %
        
        %As suggested, we replaced the dataset \textsf{youtube (YO)} by a larger dataset \textsf{socfba} (with 3M vertices and 23M edges), which is also used in \cite{li2020ordering}. The description of the dataset and the results can be found in Table~\ref{tab:data} and Fig.~\ref{subfig:a}, respectively. As expected, \texttt{EBBkC+ET} outperforms other state-of-the-art algorithms for all $k$ values. 

    
       % Besides, we used \textsf{ClueWeb09 (CW)}, \textsf{Wikipedia13 (WP)}, \textsf{AllWebUK02 (UK)} to test the scalability of our algorithms.
        %
       % We note that there are some inconsistencies on the statistics (specifically, $|V|$) of these three datasets between our paper and \cite{yuan2022efficient} (see Table~\ref{tab:data} of our paper and Table III of \cite{yuan2022efficient}). The reason is that \cite{yuan2022efficient} reports the max id of the vertices while we report the number of unique vertices. 
        %
       % We conducted the experiments following \cite{yuan2022efficient} in a parallel setting with 48 threads. The results can be found in Fig.~\ref{fig:scale}. \texttt{EBBkC+ET} can significantly improve the efficiency when $k$ is near the size of a maximum clique. Notably, on the largest graph \textsf{WP}, \texttt{EBBkC+ET} runs near two orders of magnitude faster than the state-of-the-art algorithm \texttt{BitCol} when $k=425$.
        
        

        \item[(5)] 
        We make the following clarifications on the relative performance of our method w.r.t. that of \texttt{BitCol} \cite{yuan2022efficient}.

        \underline{First}, the performance gain introduced by the two pre-processing techniques in \cite{yuan2022efficient} is not as large as that reported in the \texttt{BitCol} paper~\cite{yuan2022efficient} for two reasons. (1) The running time results reported in \cite{yuan2022efficient} do not cover the time costs of the pre-processing, as we have explained in our response to R4O1(3). (2) We checked the implementation of one of the pre-processing techniques, namely, \textit{Pre-List}, which aims to efficiently list $k$-cliques in some large cliques, as provided by the authors of \cite{yuan2022efficient}. We found that it simply counts the number of $k$-cliques in a combinatorial manner (which only needs $O(1)$ time), but does not list them (which needs $O(\tbinom{n}{k})$ time for listing $k$-cliques within $n$-cliques). 
        
        We fixed the above issues for the experiments on the \texttt{BitCol} method and found that the two pre-processing techniques do not always have their gains larger than their workloads. For example, based on the results shown in Figure~\ref{fig:variant}, on the \textsf{PO} dataset, \texttt{BitCol+} runs faster than \texttt{DDegCol+} for some settings of $k$ but slower for some other settings. Note that \texttt{BitCol+} and \texttt{DDegCol+} only differ in that the former employs the pre-processing techniques while the latter does not.
        % the DDegCol algorithm (with the pre-processing techniques), which corresponds to the \texttt{BitCol} algorithm without the SIMD-based implementations, runs a bit slower than the algorithm (without the pre-processing techniques).
        
        % \underline{Second}, based on Figure 6, our \texttt{EBBkC} framework works better than the SOTA without SIMD-based implementations, which include the DDegCol algorithm and the DDegCol algorithm with the two pre-processing techniques in the \texttt{BitCol} paper employed. 
        
        \underline{Second}, based on Figure~\ref{fig:real-small} and Figure~\ref{fig:real-large}, our \texttt{EBBkC+ET} algorithm (our complete solution), which does not involve SIMD-based implementations, works consistently better than the \texttt{BitCol} method, which includes SIMD-based implementations. We note that the performance our algorithm can be potentially boosted with SIMD-based implementations, which we leave as future work, and in this case, the performance gap between our algorithm and \texttt{BitCol} can be expected to be even larger.
        % {\yuiR
        %     We clarify that the performance of \texttt{BitCol} in our paper is consistent with that in~\cite{yuan2022efficient} in general. The possible differences come from (1) the different measurements of running time and (2) our fixation to the unfair implementation of the pre-processing method \textit{Pre-List}. Details please refer to the response to R\#4O1.(3). 
        % }
        
        %Similar to (3), we checked the source code of \cite{yuan2022efficient} and found that for \textit{Pre-List}, the implementation only counts the $k$-cliques in a clique-like connected component in a combinatorial manner (which only needs $O(1)$ time) instead of listing them (which needs $O(\tbinom{n}{k})$ time if the connected component has $n$ vertices). We fixed this issue and found that the speedup of \texttt{BitCol} is not as much as the results they reported in \cite{yuan2022efficient}.
        
        % We note that two pre-processing techniques proposed in \cite{yuan2022efficient} are covered by our edge-oriented BB framework and early-termination technique. To see this, we illustrate it one after another. \underline{For \textit{Pre-Core}}, it can be regarded as a pruning rule using size-constraint at the first branching step. For \texttt{VBBkC} algorithms, all $k$-cliques must be contained in $(k-1)$-core; thus \cite{yuan2022efficient} first reduces the graph into its $(k-1)$-core. Similarly, for \texttt{EBBkC} algorithms, all $k$-cliques must be contained in $k$-truss; thus our edge-oriented BB framework can first reduce the graph into its $k$-truss (which can be done when we generate the truss-based edge ordering). Since $k$-truss must be a subgraph of a $(k-1)$-core, our \texttt{EBBkC} framework is more powerful than \textit{Pre-Core} technique. \underline{For \textit{Pre-List}}, it is covered by our early-termination technique since if a connected component is a clique, it can also be recognized by our early-termination technique (because a clique is equivalent to a 1-plex) but not vice versa when the connected component is a $t$-plex (with $t\ge 2$). In summary, our \texttt{EBBkC} with early-termination is more powerful than the two pre-processing techniques and can reduce more time costs.   

        \item[(6)] 
        The time costs of generating the truss-based ordering for edges in \texttt{EBBkC} and those of generating the degeneracy ordering for vertices in \texttt{VBBkC} are presented in Table~\ref{tab:ordering} (newly added in the revised paper). We note that while the former are slightly larger than the latter, the overall time cost of \texttt{EBBkC} is smaller than that of \texttt{VBBkC} (as shown in Figure~\ref{fig:variant}). Furthermore, these time costs have been included when measuring the running times of the algorithms (including our \texttt{EBBkC} algorithms).
        % {\yuiR We clarify that the time costs of the truss decomposition has been included in the reported results. Details please refer to the response to R\#4O1.(3).     }
        %For all algorithms, the {\yuiR reported} running time results have included the time of generating orderings (i.e., truss-based edge ordering for \texttt{EBBkC} algorithms and degeneracy ordering for \texttt{VBBkC} algorithms). We {\yuiR also separately} report the time of generating corresponding orderings on the default datasets in Table~\ref{tab:ordering}. 
        
        \item[(7)] Thanks for the comment. In the revised paper, we use $t=2$ when $k\le \tau/2$ 
        % (where $\omega$ is the size of a maximum clique and it can be known in advance), 
        and use $t=3$ when $\tau/2 < k \le \omega$. 
        %
        The rationale is that (1) when $k$ is small, \texttt{EBBkC+ET} with a smaller $t$ runs faster and \texttt{EBBkC+ET} with $t=2$ always runs faster than that with $t=1$ (see Section~\ref{subsec:2-plex} and Section~\ref{subsec:result} (6)); (2) when $k$ is large, \texttt{EBBkC+ET} with a larger $t$ runs faster. However, since there is not a huge speedup when $t>3$ (see the results in Section~\ref{subsec:result} (6)), we choose $t=3$ as default value.
        %
        We have added the above notes in the experimental setting of Section~\ref{subsec:setup}.

        \item[(8)] 
        The running time results of Figure 10
        % in the original paper 
        % (which is still Figure~\ref{fig:parallel} in the revised paper) 
        and those of Figure 4 in the original paper (which becomes Figure~\ref{fig:parallel} and Figure~\ref{fig:real-large} in the revised paper, respectively) are consistent. They look to be inconsistent because we used different units of time, namely ``milliseconds'' in the former and ``seconds'' in the latter. In the revised paper, we use the same unit ``seconds'' in all figures.
    \end{itemize}
    \end{response}

    \smallskip
    \item[O2.] \textit{Theoretical anaylsis needs more words in actual paper.}
     % \begin{itemize}[leftmargin=*]
        % \item[(1)] 
        \textit{\underline{First}, I found the discussion around Th. 4.2. quite tight; I'd appreciate more intuition here.}
        % \item[(2)] 
        \textit{\underline{Second}, what about the cost of computing the truss-based edge ordering? The paper gives $O(m^{1.5})$ but does not include that cost in the main result.}
        % \item[(3)] 
        \textit{\underline{Third}, can anything be said about the space complexity? (The max depth of the search tree is higher than for vertex-based ordering, for instance, which requires more memory.) }

    % \end{itemize}


    \smallskip
    \begin{response}
       \begin{itemize}[leftmargin=*]

       \item[(1)] We have included more discussions on $\tau$ (including the definition, the differences between $\tau$ and graph degeneracy $\delta$, and the effects on both theoretical and practical performance of \texttt{EBBkC}) in Section~\ref{subsec:EBBkC-T}.

       \item[(2)] We note that given an integer $k\ge 3$, the time cost of generating the truss-based edge ordering, which is $O(m^{1.5})$, is dominated by the cost of the branch-and-bound search process, which is $O(km(\tau/2)^{k-2})$, under the worst case.
       % for $k\ge 3$. 
       This is because $\tau$ is tightly bounded by $\delta$ (e.g., in a complete graph, $\tau = \delta - 1$) and $\delta$ is tightly bounded by $O(\sqrt{m})$ according to the results in~\cite{barenboim2008sublogarithmic, lin2012arboricity}. Therefore, the time complexity of \texttt{EBBkC} (including the time cost of generating the truss-based edge ordering) is $O(km(\tau/2)^{k-2})$ for $k\ge 3$. We have included this clarification in Section~\ref{subsec:EBBkC-T}. We also note that the running time results of \texttt{EBBkC} reported in our experiments include those for generating the edge orderings.

       \item[(3)] The space complexity of our \texttt{EBBkC} algorithm is $O(m+n)$, which is the same as those of the existing methods. We note that the maximum depth of the search tree of the \texttt{EBBkC} algorithm is half of that of \texttt{VBBkC} algorithms since at each branching step, \texttt{EBBkC} includes two vertices while \texttt{VBBkC} includes only one vertex. We have included space complexity of our \texttt{EBBkC} algorithms in Theorem~\ref{theo:ebbkc-t}, Theorem~\ref{theo:ebbkc-c} and Theorem~\ref{theo:ebbkc-h}.
        We have reported the empirical space costs in Section~\ref{subsec:result} (8). The results show that the empirical space costs of all methods are comparable, which is consistent with our analysis.
    \end{itemize}
    \end{response}

    % \smallskip
    % \begin{response}
    %     {\yuiR Thanks for the comment. In the revision, we have included firmed theoretical results and discussions to answer your questions as follows.
        
    %     First, we have included more discussions on $\tau$ (including the definition, the differences between $\tau$ and graph degeneracy $\delta$, and the effects on both theoretical and practical performance of \texttt{EBBkC}) in Section~\ref{subsec:EBBkC-T}. More details please refer to our response to R\#2O3 and R\#3O3.
    %     }
    
    %     Second, the cost of generating the truss-based edge ordering is $O(m^{1.5})$, which is dominated by $O(km(\tau/2)^{k-2})$ when {\yuiR $k\ge 3$} since $\tau <\delta$ {\yuiR (lemma~\ref{lemma:comparison}) and $ \delta< 2\sqrt{m}$ ~\cite{barenboim2008sublogarithmic, lin2012arboricity}.} 
    %     %Besides, it is easier to make comparison with the complexity of the algorithm under vertex-oriented framework (i.e, $O(km(\tau/2)^{k-2})$ vs. $O(km(\delta/2)^{k-2})$).
    %     Hence, we omit $O(m^{1.5})$ in  Theorem~\ref{theo:ebbkc-t}. 
    %     {\yuiR We have included the above note in the proof of Theorem~\ref{theo:ebbkc-t}.}
    %     {\yuiR Besides, we would like to clarify again that the reported time includes the time costs of generating the orderings.} 
        
    %     Third, the space complexity of our \texttt{EBBkC} algorithms are $O(m+n)$, {\yuiR which are the same as the existing methods including \texttt{DDegCol} and \texttt{BitCol}.} 
    %     %Specifically, we note that (1) the maximum depth of the search tree of \texttt{EBBkC} algorithms is the half of that of \texttt{VBBkC} algorithms since at each branching step, \texttt{EBBkC} includes two vertices while \texttt{VBBkC} includes only one vertex; (2) the maximum width of the search tree of \texttt{EBBkC} algorithms is at most $|E|$ while the maximum width of the search tree of \texttt{VBBkC} algorithms is at most $|V|$. 
    %     %
    %     {\yuiR We have included the analysis of space complexity in Theorem~\ref{theo:ebbkc-t}, Theorem~\ref{theo:ebbkc-c} and Theorem~\ref{theo:ebbkc-h}.}
    %     We reported the practical memory costs in Sec~\ref{subsec:result} (8){\yuiR, and note that the memory consumption of all methods is comparable, which is consistent with our analysis.} 
    % \end{response}

\smallskip
    \item[O3.] \textit{Parallelization seems to be enough. Similar results to what's proposed in the paper can be achieved by simply using a bit more computation, as parallelization is easy to do. I don't hold this against the paper since the proposed method is also easy to parallelize and it's not overly complicated, too.}

    \smallskip
    \begin{response}
       Thanks for the comment. Our \texttt{EBBkC+ET} algorithm can be easily  parallelized. We have reported the results on the default datasets under the parallel setting in Section~\ref{subsec:result} (7). We note that our algorithm performs better than other baselines under the parallel setting.
    \end{response}

\smallskip
    \item[D1.] \textit{The discussion of Sec. 3 and 4.1 feels quite repetitive. If space is needed, that's a good place to cut.}

    \smallskip
    \begin{response}
       Thank you for the comment. Since one additional page is allowed for a revised paper, we have enough space for the newly added materials and keep Section~\ref{sec:vbbkc} and Section~\ref{subsec:motivation} unchanged. This would make it possible for those readers with some background knowledge of \texttt{VBBkC} to skip Section~\ref{sec:vbbkc} and read Section~\ref{subsec:motivation} directly.
    \end{response}

\smallskip
    \item[D2.] \textit{The paper should more clearly attribute inspiration from prior work. For example, the ``hybrid'' idea is already present in DDegCol, but that's only said in passing at the very end.
}

    \smallskip
    \begin{response}
       Thanks for the comment. We have included a note in the first paragraph of Section~\ref{subsec:EBBkC-H} to attribute the inspiration of the ``hybrid ordering'' from the existing papers including the \texttt{DDegCol} paper \cite{li2020ordering}.
    \end{response}

\smallskip
    \item[D3.] \textit{Right before (2), the paper writes ``and those vertices that disconnect the vertices incident to $e_i$'', a formulation which I find confusing. This happens at multiple places, where the paper uses ``disconnect'' when it means ``not connected'' (e.g., also when defining a $t$-plex).}

    \smallskip
    \begin{response}
    We have changed ``disconnect'' to ``is/are disconnected from''.
    \end{response}

\smallskip
    \item[D4.] \textit{Are there any downsides of EBB over VBB? Any limitations?}
    
    \smallskip
    \begin{response}
    As far as we can see, there is no major downside of EBB over VBB. A minor one is that EBB has a slightly larger space cost than VBB (as shown in Figure~\ref{fig:mem}) though they have the same space complexity.
       % {\yuiR One possible limitation is that generating ordering of edges (e.g., via truss decomposition) costs more than that of vertices (e.g., via core decomposition) since real graphs consist of more edges than vertices, as verified in Table~\ref{tab:ordering}. We have included the above note in Section~\ref{subsec:result} (1).}
    \end{response}

\smallskip
    \item[D5.] \textit{In Alg. 3, using $V[\cdot]$ and $E[\cdot]$ to means something completely different to $V(\cdot)$ and $E(\cdot)$ was highly confusing to me at first. I feel that $V[\cdot]$ and $E[\cdot]$ should be named differently to avoid such confusion.}

    \smallskip
    \begin{response}
        %Thanks for your comment.
        We have changed the notation $V[\cdot]$ and $E[\cdot]$ to $VSet(\cdot)$ and $ESet(\cdot)$, respectively, in Algorithm~\ref{alg:EBBkC-T}.
    \end{response}

\smallskip
    \item[D6.] \textit{Something like Rule (2) in Sec. 4.3 can also be used with vertex-based ordering (at least $l-1$ different colors must remain). Hasn't this been done in prior work?}

    \smallskip
    \begin{response}
       To our best knowledge, 
       % this is the first work that proposes Rule (2).
       Rule (2) is newly proposed in our paper.
       We note that Rule (2) can also be applied in \texttt{VBBkC}.
       % is orthogonal to BB frameworks including VBB and EBB. 
       We have included this note in Section~\ref{subsec:EBBkC-C}.

       Besides, we note that when conducting the ablation studies (which involve comparing between \texttt{EBBkC} and \texttt{VBBkC}) in the experiments, whose results are shown in Figure~\ref{fig:variant}, we have applied Rule (2) in both frameworks for fair comparison.
    \end{response}

\smallskip
    \item[D7.] \textit{ I found Sec. 5 to be more involved to follow, compared to the prior parts. Since this section is important for practical runtime, I suggest to spend more space, perhaps even a figure.
}

    \smallskip
    \begin{response}
    We have included a visual example in Figure~\ref{fig:t-plex} and some descriptions in Section~\ref{sec:early-termination} for a better illustration.
    \end{response}

\smallskip
    \item[D8.] \textit{The runtime results on very small graphs such as YO do not seem to be relevant.}

    \smallskip
    \begin{response}
    We have replaced in Table~\ref{tab:data} the dataset \textsf{YO} by a larger one \textsf{socfba} (used in \cite{li2020ordering}), and reported the new  results in Figure~\ref{subfig:a}. We note that \texttt{EBBkC+ET} outperforms other baselines on \textsf{socfba}, which is consistent with the results on other datasets. 
    \end{response}

\smallskip
    \item[D9.] \textit{Typos: Right before (4): ``common numbers'' to ``common neighbors''.}

    \smallskip
    \begin{response}
    We have changed ``common numbers'' to ``common neighbors''.
    \end{response}
    
\end{enumerate}

==> cover-letter/thank.tex <==


\section*{To All Reviewers}
%\label{sec:response}

\smallskip
We would like to thank you for your constructive and inspiring comments. We have gone through these comments carefully and revised our draft accordingly. %Below we summarize the major changes.
%
%\begin{enumerate}[leftmargin=*]
%\item
%\end{enumerate}
%}
%
% These major changes are highlighted in blue in the revised paper.
% Appended please find our detailed responses to both the reviewers' and meta-reviewer's comments.
% Thank you for your time reading them.
%
We highlight the major changes with the {\color{blue} blue} color in the revised manuscript. Below please find our detailed responses to all reviewers' comments. 
%We really appreciate your feedback and time.

